Learning Action and Reasoning-Centric Image Editing from Videos and Simulations

An image editing model should be able to perform diverse edits, ranging from object replacement, changing attributes or style, to performing actions or movement, which require many forms of reasoning. Current general instruction-guided editing models have significant shortcomings with action and reasoning-centric edits. Object, attribute or stylistic changes can be learned from visually static datasets. On the other hand, high-quality data for action and reasoning-centric edits is scarce and has to come from entirely different sources that cover e.g. physical dynamics, temporality and spatial reasoning. To this end, we meticulously curate the AURORA Dataset (Action-Reasoning-Object-Attribute), a collection of high-quality training data, human-annotated and curated from videos and simulation engines. We focus on a key aspect of quality training data: triplets (source image, prompt, target image) contain a single meaningful visual change described by the prompt, i.e., truly minimal changes between source and target images. To demonstrate the value of our dataset, we evaluate an AURORA-finetuned model on a new expert-curated benchmark (AURORA-Bench) covering 8 diverse editing tasks. Our model significantly outperforms previous editing models as judged by human raters. For automatic evaluations, we find important flaws in previous metrics and caution their use for semantically hard editing tasks. Instead, we propose a new automatic metric that focuses on discriminative understanding. We hope that our efforts : (1) curating a quality training dataset and an evaluation benchmark, (2) developing critical evaluations, and (3) releasing a state-of-the-art model, will fuel further progress on general image editing.

==> images/sample_outputs/figures.tex <==

        \begin{figure}[h!]
            \centering
        
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/magicbrush/0.jpg}
                \caption{Example 1}
                \label{fig:aurora_magicbrush_0}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/magicbrush/1.jpg}
                \caption{Example 2}
                \label{fig:aurora_magicbrush_1}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/magicbrush/2.jpg}
                \caption{Example 3}
                \label{fig:aurora_magicbrush_2}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/magicbrush/3.jpg}
                \caption{Example 4}
                \label{fig:aurora_magicbrush_3}
            \end{subfigure}
            
            \caption{Comparison for magicbrush task}
            \label{fig:aurora_magicbrush}
        \end{figure}
        \newpage
        
        \begin{figure}[h!]
            \centering
        
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/magicbrush/0.jpg}
                \caption{Example 1}
                \label{fig:magicbrush_magicbrush_0}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/magicbrush/1.jpg}
                \caption{Example 2}
                \label{fig:magicbrush_magicbrush_1}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/magicbrush/2.jpg}
                \caption{Example 3}
                \label{fig:magicbrush_magicbrush_2}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/magicbrush/3.jpg}
                \caption{Example 4}
                \label{fig:magicbrush_magicbrush_3}
            \end{subfigure}
            
            \caption{Comparison for magicbrush task}
            \label{fig:magicbrush_magicbrush}
        \end{figure}
        \newpage
        
        \begin{figure}[h!]
            \centering
        
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/something/0.jpg}
                \caption{Example 1}
                \label{fig:aurora_something_0}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/something/1.jpg}
                \caption{Example 2}
                \label{fig:aurora_something_1}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/something/2.jpg}
                \caption{Example 3}
                \label{fig:aurora_something_2}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/something/3.jpg}
                \caption{Example 4}
                \label{fig:aurora_something_3}
            \end{subfigure}
            
            \caption{Comparison for something task}
            \label{fig:aurora_something}
        \end{figure}
        \newpage
        
        \begin{figure}[h!]
            \centering
        
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/something/0.jpg}
                \caption{Example 1}
                \label{fig:magicbrush_something_0}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/something/1.jpg}
                \caption{Example 2}
                \label{fig:magicbrush_something_1}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/something/2.jpg}
                \caption{Example 3}
                \label{fig:magicbrush_something_2}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/something/3.jpg}
                \caption{Example 4}
                \label{fig:magicbrush_something_3}
            \end{subfigure}
            
            \caption{Comparison for something task}
            \label{fig:magicbrush_something}
        \end{figure}
        \newpage
        
        \begin{figure}[h!]
            \centering
        
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/ag/0.jpg}
                \caption{Example 1}
                \label{fig:aurora_ag_0}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/ag/1.jpg}
                \caption{Example 2}
                \label{fig:aurora_ag_1}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/ag/2.jpg}
                \caption{Example 3}
                \label{fig:aurora_ag_2}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/ag/3.jpg}
                \caption{Example 4}
                \label{fig:aurora_ag_3}
            \end{subfigure}
            
            \caption{Comparison for ag task}
            \label{fig:aurora_ag}
        \end{figure}
        \newpage
        
        \begin{figure}[h!]
            \centering
        
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/ag/0.jpg}
                \caption{Example 1}
                \label{fig:magicbrush_ag_0}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/ag/1.jpg}
                \caption{Example 2}
                \label{fig:magicbrush_ag_1}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/ag/2.jpg}
                \caption{Example 3}
                \label{fig:magicbrush_ag_2}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/ag/3.jpg}
                \caption{Example 4}
                \label{fig:magicbrush_ag_3}
            \end{subfigure}
            
            \caption{Comparison for ag task}
            \label{fig:magicbrush_ag}
        \end{figure}
        \newpage
        
        \begin{figure}[h!]
            \centering
        
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/kubric/0.jpg}
                \caption{Example 1}
                \label{fig:aurora_kubric_0}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/kubric/1.jpg}
                \caption{Example 2}
                \label{fig:aurora_kubric_1}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/kubric/2.jpg}
                \caption{Example 3}
                \label{fig:aurora_kubric_2}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/kubric/3.jpg}
                \caption{Example 4}
                \label{fig:aurora_kubric_3}
            \end{subfigure}
            
            \caption{Comparison for kubric task}
            \label{fig:aurora_kubric}
        \end{figure}
        \newpage
        
        \begin{figure}[h!]
            \centering
        
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/kubric/0.jpg}
                \caption{Example 1}
                \label{fig:magicbrush_kubric_0}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/kubric/1.jpg}
                \caption{Example 2}
                \label{fig:magicbrush_kubric_1}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/kubric/2.jpg}
                \caption{Example 3}
                \label{fig:magicbrush_kubric_2}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/kubric/3.jpg}
                \caption{Example 4}
                \label{fig:magicbrush_kubric_3}
            \end{subfigure}
            
            \caption{Comparison for kubric task}
            \label{fig:magicbrush_kubric}
        \end{figure}
        \newpage
        
        \begin{figure}[h!]
            \centering
        
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/whatsup/0.jpg}
                \caption{Example 1}
                \label{fig:aurora_whatsup_0}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/whatsup/1.jpg}
                \caption{Example 2}
                \label{fig:aurora_whatsup_1}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/whatsup/2.jpg}
                \caption{Example 3}
                \label{fig:aurora_whatsup_2}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/whatsup/3.jpg}
                \caption{Example 4}
                \label{fig:aurora_whatsup_3}
            \end{subfigure}
            
            \caption{Comparison for whatsup task}
            \label{fig:aurora_whatsup}
        \end{figure}
        \newpage
        
        \begin{figure}[h!]
            \centering
        
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/whatsup/0.jpg}
                \caption{Example 1}
                \label{fig:magicbrush_whatsup_0}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/whatsup/1.jpg}
                \caption{Example 2}
                \label{fig:magicbrush_whatsup_1}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/whatsup/2.jpg}
                \caption{Example 3}
                \label{fig:magicbrush_whatsup_2}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/whatsup/3.jpg}
                \caption{Example 4}
                \label{fig:magicbrush_whatsup_3}
            \end{subfigure}
            
            \caption{Comparison for whatsup task}
            \label{fig:magicbrush_whatsup}
        \end{figure}
        \newpage
        
        \begin{figure}[h!]
            \centering
        
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/clevr/0.jpg}
                \caption{Example 1}
                \label{fig:aurora_clevr_0}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/clevr/1.jpg}
                \caption{Example 2}
                \label{fig:aurora_clevr_1}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/clevr/2.jpg}
                \caption{Example 3}
                \label{fig:aurora_clevr_2}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/clevr/3.jpg}
                \caption{Example 4}
                \label{fig:aurora_clevr_3}
            \end{subfigure}
            
            \caption{Comparison for clevr task}
            \label{fig:aurora_clevr}
        \end{figure}
        \newpage
        
        \begin{figure}[h!]
            \centering
        
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/clevr/0.jpg}
                \caption{Example 1}
                \label{fig:magicbrush_clevr_0}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/clevr/1.jpg}
                \caption{Example 2}
                \label{fig:magicbrush_clevr_1}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/clevr/2.jpg}
                \caption{Example 3}
                \label{fig:magicbrush_clevr_2}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/clevr/3.jpg}
                \caption{Example 4}
                \label{fig:magicbrush_clevr_3}
            \end{subfigure}
            
            \caption{Comparison for clevr task}
            \label{fig:magicbrush_clevr}
        \end{figure}
        \newpage
        
        \begin{figure}[h!]
            \centering
        
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/epic/0.jpg}
                \caption{Example 1}
                \label{fig:aurora_epic_0}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/epic/1.jpg}
                \caption{Example 2}
                \label{fig:aurora_epic_1}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/epic/2.jpg}
                \caption{Example 3}
                \label{fig:aurora_epic_2}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/epic/3.jpg}
                \caption{Example 4}
                \label{fig:aurora_epic_3}
            \end{subfigure}
            
            \caption{Comparison for epic task}
            \label{fig:aurora_epic}
        \end{figure}
        \newpage
        
        \begin{figure}[h!]
            \centering
        
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/epic/0.jpg}
                \caption{Example 1}
                \label{fig:magicbrush_epic_0}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/epic/1.jpg}
                \caption{Example 2}
                \label{fig:magicbrush_epic_1}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/epic/2.jpg}
                \caption{Example 3}
                \label{fig:magicbrush_epic_2}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/epic/3.jpg}
                \caption{Example 4}
                \label{fig:magicbrush_epic_3}
            \end{subfigure}
            
            \caption{Comparison for epic task}
            \label{fig:magicbrush_epic}
        \end{figure}
        \newpage
        
        \begin{figure}[h!]
            \centering
        
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/emu/0.jpg}
                \caption{Example 1}
                \label{fig:aurora_emu_0}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/emu/1.jpg}
                \caption{Example 2}
                \label{fig:aurora_emu_1}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/emu/2.jpg}
                \caption{Example 3}
                \label{fig:aurora_emu_2}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/aurora/emu/3.jpg}
                \caption{Example 4}
                \label{fig:aurora_emu_3}
            \end{subfigure}
            
            \caption{Comparison for emu task}
            \label{fig:aurora_emu}
        \end{figure}
        \newpage
        
        \begin{figure}[h!]
            \centering
        
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/emu/0.jpg}
                \caption{Example 1}
                \label{fig:magicbrush_emu_0}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/emu/1.jpg}
                \caption{Example 2}
                \label{fig:magicbrush_emu_1}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/emu/2.jpg}
                \caption{Example 3}
                \label{fig:magicbrush_emu_2}
            \end{subfigure}
            
            \begin{subfigure}[b]{0.24\textwidth}
                \centering
                \includegraphics[width=\textwidth]{evaluation/sample_outputs/magicbrush/emu/3.jpg}
                \caption{Example 4}
                \label{fig:magicbrush_emu_3}
            \end{subfigure}
            
            \caption{Comparison for emu task}
            \label{fig:magicbrush_emu}
        \end{figure}
        \newpage
        

==> itm_table.tex <==
\begin{table*}
\small
\centering
\caption{DiscEdit performance (\Cref{subsec:disc} comparing the two strongest models from human judgement \Cref{tab:human_eval}. We show binary accuracy with a 50\% random baseline. Details: we average each example over 4 noise samples for the denoising diffusion process.}
\begin{tabular}{@{}lccccc@{}}
\toprule
\textbf{Model} & \textbf{WhatsUp} & \textbf{Something} & \textbf{AG} & \textbf{Kubric} & \textbf{CLEVR} \\
\midrule
\textbf{MagicBrush} & 0.472 & 0.530 & 0.339 & 0.439 & 0.188 \\
\textbf{Ours} & 0.561 & 0.507 & 0.548 & 0.606 & 0.562 \\
\bottomrule
\end{tabular}
\label{tab:finetuning}
\vspace{-1em}
\end{table*}

==> itm_table_extended.tex <==
\begin{table*}[!ht]
\small
\centering
\caption{\textbf{L2 Latent}: EditITM method on our discriminative benchmark with 400 instruction-pairs differing in minimal ways, across three datasets. Performance in binary accuracy with a 50\% random baseline. Details: we average each example over 8 samples from the diffusion process.}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\textbf{Model} & \multicolumn{6}{c}{\textbf{Handcrafted-EditITM (Flickr30K)}} & \multicolumn{1}{c}{\textbf{SVO}} & \multicolumn{1}{c}{\textbf{WhatsUp}} \\
\cmidrule(lr){2-7}
 & \textbf{ALL} & \textbf{Action} & \textbf{Attribute} & \textbf{Global} & \textbf{Remove} & \textbf{Referring} &  &  \\

\midrule

\textbf{GenHowTo} &  &  &  &  &  &  &  &  \\

\textbf{MGIE} &  &  &  &  &  &  &  &  \\

\textbf{InstructPix2Pix} &  &  &  &  &  &  &  &  \\

\textbf{MagicBrush} & 0.618 & 0.5 & 0.723 & 0.682 & 0.58 & 0.597 & 0.706 & 0.515 \\

\textbf{MagicBrush-copy0.2} & 0.59 & 0.457 & 0.708 & 0.697 & 0.568 & 0.565 & 0.706 & 0.62  \\

\textbf{Ours} & 0.61 & 0.5 & 0.723 & 0.591 & 0.63 & 0.597 & 0.529 & 0.509 \\

\textbf{Ours-copy0.2} &  &  &  &  &  &  &  &  \\

\bottomrule
\end{tabular}
\label{tab:finetuning}
\vspace{-1em}
\end{table*}

\begin{table*}[!ht]
\small
\centering
\caption{\textbf{CLIP Cosine:} EditITM method on our discriminative benchmark with 400 instruction-pairs differing in minimal ways, across three datasets. Performance in binary accuracy with a 50\% random baseline. Details: we average each example over 8 samples from the diffusion process.}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\textbf{Model} & \multicolumn{6}{c}{\textbf{Handcrafted-EditITM (Flickr30K)}} & \multicolumn{1}{c}{\textbf{SVO}} & \multicolumn{1}{c}{\textbf{WhatsUp}} \\
\cmidrule(lr){2-7}
 & \textbf{ALL} & \textbf{Action} & \textbf{Attribute} & \textbf{Global} & \textbf{Remove} & \textbf{Referring} &  &  \\

\midrule

\textbf{GenHowTo} &  &  &  &  &  &  &  &  \\

\textbf{MGIE} &  &  &  &  &  &  &  &  \\

\textbf{InstructPix2Pix} &  &  &  &  &  &  &  &  \\

\textbf{MagicBrush} & 0.58 & 0.507 & 0.638 & 0.742 & 0.494 & 0.565 & 0.647 & 0.505 \\

\textbf{MagicBrush-copy0.2} & 0.583 & 0.442 & 0.677 & 0.833 & 0.519 & 0.484 & 0.471 & 0.59 \\

\textbf{Ours} & 0.59 & 0.551 & 0.623 & 0.652 & 0.58 & 0.484 & 0.529 & 0.548 \\

\textbf{Ours-copy0.2} &  &  &  &  &  &  &  &  \\

\bottomrule
\end{tabular}
\label{tab:finetuning}
\vspace{-1em}
\end{table*}


\begin{table*}[!ht]
\small
\centering
\caption{\textbf{L2 Latent (4 samples):} EditITM method on our discriminative benchmark with 400 instruction-pairs differing in minimal ways, across three datasets. Performance in binary accuracy with a 50\% random baseline. Details: we average each example over 8 samples from the diffusion process.}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\textbf{Model} & \multicolumn{6}{c}{\textbf{Handcrafted-EditITM (Flickr30K)}} & \multicolumn{1}{c}{\textbf{SVO}} & \multicolumn{1}{c}{\textbf{WhatsUp}} \\
\cmidrule(lr){2-7}
 & \textbf{ALL} & \textbf{Action} & \textbf{Attribute} & \textbf{Global} & \textbf{Remove} & \textbf{Referring} &  &  \\

\midrule

\textbf{GenHowTo} &  &  &  &  &  &  &  &  \\

\textbf{MGIE} &  &  &  &  &  &  &  &  \\

\textbf{InstructPix2Pix} &  &  &  &  &  &  &  &  \\

\textbf{MagicBrush} & 0.62 & 0.493 & 0.715 & 0.682 & 0.617 & 0.565 & 0.765 & 0.501  \\

\textbf{MagicBrush-copy0.2} &0.603 & 0.478 & 0.715 & 0.742 & 0.556 & 0.548 & 0.706 & 0.585  \\

\textbf{Ours} & 0.595 & 0.471 & 0.723 & 0.561 & 0.63 & 0.597 & 0.471 & 0.516  \\

\textbf{Ours-copy0.2} &  &  &  &  &  &  &  &  \\

\bottomrule
\end{tabular}
\label{tab:finetuning}
\vspace{-1em}
\end{table*}



\begin{table*}[!ht]
\small
\centering
\caption{\textbf{L2 Latent (1 sample):} EditITM method on our discriminative benchmark with 400 instruction-pairs differing in minimal ways, across three datasets. Performance in binary accuracy with a 50\% random baseline. Details: we average each example over 8 samples from the diffusion process.}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\textbf{Model} & \multicolumn{6}{c}{\textbf{Handcrafted-EditITM (Flickr30K)}} & \multicolumn{1}{c}{\textbf{SVO}} & \multicolumn{1}{c}{\textbf{WhatsUp}} \\
\cmidrule(lr){2-7}
 & \textbf{ALL} & \textbf{Action} & \textbf{Attribute} & \textbf{Global} & \textbf{Remove} & \textbf{Referring} &  &  \\

\midrule

\textbf{GenHowTo} &  &  &  &  &  &  &  &  \\

\textbf{MGIE} &  &  &  &  &  &  &  &  \\

\textbf{InstructPix2Pix} &  &  &  &  &  &  &  &  \\

\textbf{MagicBrush} & 0.627 & 0.507 & 0.708 & 0.727 & 0.63 & 0.548 & 0.765 & 0.492  \\

\textbf{MagicBrush-copy0.2} & 0.583 & 0.42 & 0.685 & 0.727 & 0.617 & 0.548 & 0.706 & 0.585  \\

\textbf{Ours} & 0.588 & 0.464 & 0.662 & 0.621 & 0.679 & 0.548 & 0.471 & 0.513  \\

\textbf{Ours-copy0.2} &  &  &  &  &  &  &  &  \\

\bottomrule
\end{tabular}
\label{tab:finetuning}
\vspace{-1em}
\end{table*}



